Cryptographically Assured Information Flow: Assured Remote Execution

Assured Remote Execution on a device is the ability of suitably authorized parties to construct secure channels with known processes -- i.e. processes executing known code -- running on it. Assured Remote Execution requires a hardware basis including cryptographic primitives. In this paper, we show that a simple hardware-level mechanism called Cryptographically Assured Information Flow (CAIF) enables Assured Remote Execution. CAIF is akin to some operations in existing Trusted Execution Environments, but securely implements an ideal functionality defined in terms of logging and confidential escrow. We show how to achieve Assured Remote Execution for a wide variety of processes on a CAIF device. Cryptographic protocol analysis demonstrates our security goals are achieved even against a strong adversary that may modify our programs and execute unauthorized programs on the device. Assured Remote Execution enables useful functionality such as trustworthy remote attestation, and provides some of the support needed for secure remote reprogramming.

==> adversary.tex <==
In this section, we describe our adversary, and then show how to model
the adversary formally.  We then formalize the delegation protocol
from {\S\,}\ref{sec:delegation}, after which we turn to the symmetric
anchoring protocol of {\S\,}\ref{sec:anchoring:ss}.  The asymmetric
method of {\S\,}\ref{sec:anchoring:ds} raises no interesting
challenge.







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "arex"
%%% End:

